DyFo: A Training-Free Dynamic Focus Visual Search for Enhancing LMMs in Fine-Grained Visual Understanding

Humans can effortlessly locate desired objects in cluttered environments, relying on a cognitive mechanism known as visual search to efficiently filter out irrelevant information and focus on task-related regions. Inspired by this process, we propose Dyfo (Dynamic Focus), a training-free dynamic focusing visual search method that enhances fine-grained visual understanding in large multimodal models (LMMs). Unlike existing approaches which require additional modules or data collection, Dyfo leverages a bidirectional interaction between LMMs and visual experts, using a Monte Carlo Tree Search (MCTS) algorithm to simulate human-like focus adjustments. This enables LMMs to focus on key visual regions while filtering out irrelevant content, without introducing additional training caused by vocabulary expansion or the integration of specialized localization modules. Experimental results demonstrate that Dyfo significantly improves fine-grained visual understanding and reduces hallucination issues in LMMs, achieving superior performance across both fixed and dynamic resolution models. The code is available at https://github.com/PKU-ICST-MIPL/DyFo_CVPR2025

==> tables/vstar.tex <==
\begin{table*}[h]
\centering
\resizebox{0.825\linewidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
\multirow{2}{*}{Model}        & \multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{Attribute}}                                   & \multicolumn{2}{c}{\textbf{Spatial}}                               & \multicolumn{1}{c}{\multirow{2}{*}{Total Scores$\uparrow$}} \\
                              &                           & \multicolumn{1}{c}{\textit{Accuracy}$\uparrow$} & \multicolumn{1}{c}{\textit{F1 Score}$\uparrow$} & \multicolumn{1}{c}{\textit{Accuracy}$\uparrow$} & \multicolumn{1}{c}{\textit{F1 Score}$\uparrow$} & \multicolumn{1}{c}{}                       \\ \midrule
\multirow{5}{*}{LLaVA1.5}     & \rowcolor{gray!30} Regular                   
                              & $37.39$ & $32.15$ & $39.47$ & $34.97$ &$38.22$ \\
                              & ZS-CoT (NeurIPS 2022)                      & & & & & \\
                              & CCoT (CVPR 2024)
                              & & & & & \\
                              & VCD (CVPR 2024)                     
                              & & & & & \\
                              & \ourmethod (Ours)                    
                              & & & &  & \textbf{54.97} \\
                              \midrule
\multirow{5}{*}{Qwen2-VL*}     & \rowcolor{gray!30} Regular                   
                              & $33.04$ & $0.3261$ & $57.89$ & $58.03$ &$42.93$ \\
                              & ZS-CoT (NeurIPS 2022)                      & & & & & \\
                              & CCoT (CVPR 2024)
                              & & & & & \\
                              & VCD (CVPR 2024)                     
                              & & & & & \\
                              & \ourmethod  (Ours)                     
                              & & & &  & \textbf{63.35} \\
                              \midrule
\multirow{5}{*}{Qwen2-VL}     & \rowcolor{gray!30} Regular                   
                              & $74.78$ & $74.17$ & $68.42$ & $67.86$ &$72.25$ \\
                              & ZS-CoT (NeurIPS 2022)                      & & & & & \\
                              & CCoT (CVPR 2024)
                              & & & & & \\
                              & VCD (CVPR 2024)                     
                              & & & & & \\
                              & \ourmethod   (Ours)                    
                              & & & & & \textbf{73.30} \\
                              \bottomrule
\end{tabular}
}
\caption{Results on V* Bench. "Regular" refers to LMMs generating answers directly, while \ourmethod indicates using our method for visual search before answering, compared with other training-free LMM enhancement techniques, including Zero-shot CoT (ZS-CoT), CCoT, and VCD. The best performances within each setting are \textbf{bolded}.}
\label{tab:vstar}
%\vspace{-0.2cm}
\end{table*}
